Learning to Optimize Energy Efficiency in Energy Harvesting Wireless Sensor Networks

We study wireless power transmission by an energy source to multiple energy harvesting nodes with the aim to maximize the energy efficiency. The source transmits energy to the nodes using one of the available power levels in each time slot and the nodes transmit information back to the energy source using the harvested energy. The source does not have any channel state information and it only knows whether a received codeword from a given node was successfully decoded or not. With this limited information, the source has to learn the optimal power level that maximizes the energy efficiency of the network. We model the problem as a stochastic Multi-Armed Bandits problem and develop an Upper Confidence Bound based algorithm, which learns the optimal transmit power of the energy source that maximizes the energy efficiency. Numerical results validate the performance guarantees of the proposed algorithm and show significant gains compared to the benchmark schemes.

==> Energy Harvesting_Problem/algorithm.tex <==
We develop an algorithm for optimal power selection using the well known UCB approach \cite{lattimore2020bandit}. We begin by giving a concentration bound on the sum of weighted random variables that will be used in the algorithm.  Let $\hat\mu_{ij}^{(s)}$ denote the empirical mean obtained from $s$ i.i.d. samples of the received rate at the source from node $j$ using the energy harvested from power $i$, given by $\hat\mu_{ij}^{(s)}=\frac{1}{s}\sum_{t=1}^sR_j^i(t)$.
Since $R_j^i(t)\in \{0,r_0\}$, by Hoeffding's Lemma \cite[eq. (2.2)]{book2012_bubeck_regret} there exits a convex function $\psi:\mathbb{R}\rightarrow \mathbb{R}_+$ such that for all $a > 0$,
 \begin{align}
  \EE{\exp(a(\mu_{ij}-R_j^i))} \leq \exp(\psi(a)),\label{eqn:Hoeffding lemma}
  %\shortintertext{where the convex function $\psi(a)=a^2r_0^2/8$.} \nonumber
 \end{align}
where the convex function $\psi(a)=a^2r_0^2/8$. %In this case, equation \eqref{eqn:Hoeffding lemma} is known as Hoeffiding's lemma.

Using \eqref{eqn:Hoeffding lemma} we get the following concentration bound on the weighted sum rate received at the source.
\begin{lem}
 \label{lem:ConcentrationBound1}
 For any $s$, we have 
 \begin{align}
\Prob{\sum\limits_{j=1}^{k}\omega_j\mu_{ij} - \sum\limits_{j=1}^{k}\omega_j\hat{\mu}_{ij}^{(s)}> \epsilon} \leq \exp(-s\psi^*(\epsilon)),\nonumber
 %\vspace{-5mm}
%\intertext{where $\psi^*(\epsilon)=\sup_{\alpha \in \mathcal{R}} (\alpha\epsilon - \sum_{j=1}^{k}\omega_j^2\psi(\alpha))$ is the (weighted) Legendre-Fenchel transform of $\psi(\alpha)$.}\nonumber% and $0 \leq \omega_j \leq 1, \forall j$, such that $\sum\limits_{j=1}^k\omega_j = 1$.}\nonumber
\end{align}% $\psi(x) = \frac{x^2r_0^2}{8}$.
 where $\psi^*(\epsilon)=\sup_{a \in \mathbb{R}} (\alpha\epsilon - \sum_{j=1}^{k}\omega_j^2\psi(a))$ is the (weighted) Legendre-Fenchel transform of $\psi(\alpha)$.
\end{lem}
\textit{Proof:} Please refer to Appendix A.

%\vspace{-8mm}
Lemma \ref{lem:ConcentrationBound1} states that with probability $1-\delta$, $\sum_{j=1}^k\omega_j\hat{\mu}^{(s)}_{ij} + (\psi^*)^{-1}\left(\frac{1}{s}\log \frac{1}{\delta}\right) > \sum_{j=1}^k\omega_j\mu_{ij}$ holds $\forall i\in m.$ % \{1,2,\dots, m\}$. % where $i = 1,2, \dots, m$.
%\begin{align}
%\label{eqn:ConfidenceInterval1}
%\sum_{j=1}^k\hat{\mu}^{(s)}_{i,j} + k (\psi^*)^{-1}\left(\frac{1}{sk}\log \frac{1}{\delta}\right) > \sum_{j=1}^k\mu_{i,j},\\
%\intertext{where $i = 1,2, \dots, m$.} \nonumber
%\end{align}
%\vspace{-4mm}
Using this lemma we define UCB for each power $i$ in time slot $t > m$ as
%\vspace{-3mm}
\begin{align}
\label{eqn:UCB2}
\mbox{UCB}_{i}(t)=\sum\limits_{j=1}^k\omega_j\hat\mu_{ij}(t-1) + (\psi^*)^{-1}\left (\frac{\alpha \ln t}{N_{i}(t-1)}\right),
%\vspace{-5mm}
\end{align}
where $\alpha$ is an input parameter to the algorithm, $N_i(t) = \sum_{s=1}^{t}\mathbb{I}\{I_s = i\}$ denotes the number of times the power $i$ is selected till time slot $t$ and $(\psi^{*})^{-1}\left(\frac{\alpha \ln t}{N_{i}(t-1)}\right)= r_{0}\sqrt{\frac{\alpha \ln t\sum_{j=1}^{k}\omega_j^2}{2N_{i}(t-1)}}$. The larger the value of $\alpha$, more is the exploration. We propose a UCB based algorithm whose pseudo-code is given in Algorithm: \ref{alg:UCB}, which 
% We develop an algorithm named \ref{alg:MaxMin-UCB} that adapt the standard UCB algorithm \cite{ML2002_FiniteTimeAnlaysis_Auer} to our setting. Recall that in our setup playing a channel gives feedback from all the nodes. Let $i\in[m]$ and $j\in [p]$, and $\hat{\mu}_{ij}(t-1)$ denote the empirical mean for the $(i,j)$ channel-node pair based on the samples observed till time $t-1$. Define $\hat{\mu}_i(t-1)= \min\limits_{j\in [p]}\hat{\mu}_i(t-1)$. We treat $\hat{\mu}_i$ as the proxy for the estimate of channel $i$ and apply the standard UCB algorithm. We refer our our algorithm as \ref{alg:MaxMin-UCB} and its pesudo-code is given in \ref{alg:MaxMin-UCB}.
works as follows. The \ref{alg:UCB} algorithm takes $m$ powers, $k$ nodes, and $\alpha$ as inputs, where $\alpha$ is a constant to be specified later. In the first $m$ time slots, each power is selected in a round-robin fashion. In each of the subsequent time slot $t$, the UCB value of power $i$ is calculated as per (\ref{eqn:UCB2}). The source then selects the power index $i$ which maximizes the ratio $\text{UCB}_i(t)/p_i$. The maximizing power index is denoted by $I_t$ and the transmit power by $p_{I_t}$. For the selected $I_t$, the source then observes the received rates $R_j^{I_t}(t)$ and updates the empirical means $\hat{\mu}_{I_tj}(t)$ for all of the nodes.
\vspace{-2mm}
\begin{algorithm}[H] 
	\renewcommand{\thealgorithm}{UCB-EH}
	\floatname{algorithm}{}
	\caption{\bf }
	\label{alg:UCB}
	\begin{algorithmic}[1]
		\STATE \textbf{Input:} $m, k, \alpha \text{ and } \omega_j, \forall j$
		\STATE Select each transmit power once in first $m$ time slots
		\STATE Update $\hat{\mu}_{ij}$ for all $i\in m, j\in k$
		\FOR{$t= m+1, m+2,\ldots, n$}
			\STATE For each power $i\in m$ calculate 
				\begin{align*}
			\text{UCB}_{i}(t)  \leftarrow \sum\limits_{j=1}^{k}\omega_j\hat\mu_{ij}(t-1) + r_{0}\sqrt{\frac{\alpha \ln t\sum_{j=1}^{k}\omega_j^2}{2N_{i}(t-1)}}	
			\end{align*}
			\STATE Set $I_{t} \leftarrow \argmax\limits_{i}\frac{\text{UCB}_{i}(t)}{p_i}$ and transmit power $p_{I_t}$
		    %\STATE Transmit power $p_{I_t}$ 
            \STATE Observe  received rate $R_{j}^{I_t}(t)$ for all $j\in k$ 
            \STATE  Update the estimates of $\hat{\mu}_{I_tj}(t)$ for all $j \in k$
		\ENDFOR
	\end{algorithmic}
\end{algorithm}
%\vspace{-10mm}
%The argmax value returns the arm i index such that in each round, an index algorithm selects the arm that maximizes the upper confidence bounds, that depends only on the current time step and the samples from that arm. Suppose the first arm at the beginning of the round t was played a lot more often than the others. If we did a good job of designing our algorithm, we would hope that this is the optimum arm, and because it's been played so often we expect $\hat{\mu}_{1j^{*}}(t-1) = \min\limits_{j \in [p]}\hat{\mu}_{1j}(t-1) \approx \mu_{1j^{*}}$
%In order to confirm the hypothesis that arm 1 is optimal, the algorithm is better to be sure that other arms are actually worse. This naturally leads to the idea of using upper boundaries of confidence. 
%The learner can be reasonably sure that arm i is worse than arm 1 if - 
%$\min\limits_{j \in [p]}\hat{\mu}_{ij}(t-1) + \sqrt{\frac{2\log(1/\delta)}{T_{i}(t-1)}} \leq \mu_{1j^{*}} \approx \min\limits_{j\in [p]}\hat{\mu}_{1j^{*}}(t-1) + \sqrt{\frac{2\log(1/\delta)}{T_{1}(t-1)}}$
\vspace{-6mm}
\subsection{Regret Analysis}
%The regret for any policy $\pi$ can be decomposed as  $\Regret_{n} = \sum\limits_{i \in M}\Delta_{i}\EE{N_{i}(n)}$, where $\Delta_{i} = \mu_{i^{*}}- \sum\limits_{j=1}^{J}\frac{\mu_{i,j}}{p_{i}}$, called as the sub-optimality gap. 
%According to the Regret Decomposition Lemma \cite{Book19_Tor19Bandits}, 
%\begin{lem}{Regret Decomposition Lemma :}
%\label{Regret Decomposition Lemma}
%the regret $\Regret_{n}$ for any policy $\pi$ satisfies
    %\begin{align}
        %$\Regret_{n} = \sum_{i=1}^{m}\Delta_{i}\EE{N_{i}(n)}$, where $N_i(n)$ denotes the number of times power $i$ is selected during $n$ time slots and $\Delta_{i} = \mu_{i^{*}}- \sum_{j=1}^{k}\frac{\mu_{ij}}{p_{i}}$ is the sub-optimality gap or immediate regret of action taken of each $i^{th}$ transmit power.
%    \end{align}
%\end{lem}
%\vspace{-2mm}
Now we give a theoretical guarantee on the performance of the proposed \ref{alg:UCB} algorithm. %All proofs of lemma and theorems can be found in Appendix. %\ref{sec:appendix}.
\begin{thm}
    \label{thm: Theorem 1}
    Let $\Delta_{i} = \mu_{i^{*}}- \sum_{j=1}^{k}(\omega_j\mu_{ij}/p_{i})$ be the sub-optimality gap of power $i$ and $\Delta = \min\limits_{i \neq i^{*}}\Delta_{i}$. Then, the regret of \ref{alg:UCB} after $n$ rounds is upper bounded as
	\begin{align}
	\label{regret:Thm1}
	    \hspace{-3mm}\Regret_{n} &\leq 6r_{o}^2\sum\limits_{i: \Delta_{i}>0}\frac{\ln n\sum_{j=1}^{k}\omega_j^2}{p_i^2\Delta_{i}} + \sum\limits_{i: \Delta_{i}>0}\left(\frac{\pi^{2}}{3} + 1\right)\Delta_{i},
	    %\intertext{i.e., the regret is upper bounded by}
	    %\Regret_{n} &\leq O\left(\frac{m \ln n\sum_{j=1}^{k}\omega_j^2}{\Delta}\right), \quad \text{where  \nonumber $\Delta = \min\limits_{i \neq i^{*}}\Delta_{i}$}
	 \end{align}
i.e., the regret is of the order $O\left(\frac{m \ln n\sum_{j=1}^{k}\omega_j^2}{\Delta}\right)$.
Further, the problem independent bound is given as $\Regret_{n} \leq O\left(\sqrt{nm\ln  n\sum_{j=1}^{k}\omega_j^2}\right).$
%\sqrt{n(m-1)\left\{6r_{0}^{2}\ln n\sum_{j=1}^{k}\omega_j^2  + r_{0}^{2}\left(\frac{\pi^{2}}{3} + 1\right)\right\}}\].
\end{thm}
\textit{Proof:} Please refer to Appendix A.

As seen from Theorem \ref{thm: Theorem 1}, the proposed UCB-EH algorithm is asymptotically optimal and thereby maximizes the expected EE. Moreover, the complexity of the proposed algorithm grows linearly with the number of power levels $m$.
%\vspace{-1mm}
\begin{comment}
%\vspace{2mm}
Next we give a problem independent upper bound on the regret.
\begin{thm}
    \label{thm: Theorem 2}
    Let \ref{alg:UCB} run for $n$ time slots. Then the regret of \ref{alg:UCB} for any instance is upper bounded by 
	\begin{align}
	\label{regret:Thm2}
	    %\Regret_{n}  \leq \sqrt{\frac{6kr_{0}^{2}(m-1)n}{p_i}\ln n  + r_{0}^{2}n(m-1)(\frac{\pi^{2}}{3} + 1)}  = O(\sqrt{knm\log n}) 
	    \hspace{-2mm}\Regret_{n} \leq \sqrt{n(m-1)\left\{6r_{0}^{2}\ln n\sum_{j=1}^{k}\omega_j^2  + r_{0}^{2}\left(\frac{\pi^{2}}{3} + 1\right)\right\}}.
	    %&= O(\sqrt{nmk\log n}) 
	\end{align}
\end{thm}
\vspace{-2mm}
\textit{Proof:} Please refer to the Appendix A.
\end{comment}
%\vspace{-8mm}
%Note that both of the above bounds depends on the number of nodes $k$, number of transmit powers $m$ and the minimum sub-optimality gap $\Delta$.

==> Energy Harvesting_Problem/conclusion.tex <==
We investigated the problem of optimal power selection at a dedicated source that wirelessly charges EH nodes in a %wirelessly powered communication network 
WPCN, for improving the EE of the system without any CSI knowledge. To address this problem, we proposed an online learning approach based on the theory of multi-armed bandit that selects the optimal transmit power which maximizes the EE of the system. %We developed an UCB based algorithm that can learn the optimal power that maximizes the energy efficiency optimization. 
The simulation results shows that the proposed algorithm learns the optimal power and it significantly outperforms the benchmark schemes. % where the source always transmits with the maximum power to charge the EH nodes.



==> Energy Harvesting_Problem/experiment.tex <==
Assuming Rayleigh fading, %and each (i,j) power-node pair has the received rate %$R_j(t)$ in \eqref{eqn: received rate} 
%with mean $\mu_{ij}$ that can be computed by evaluating the probability of success of $O_j(t)$ in \eqref{eq_O} for $P(t-1)=i$ in time slot $t$. 
%$O_j(t)$ in \eqref{eq_O}, in time slot $t$, is a Bernoulli distributed RV with the probability of success given by 
%\begin{align}
%        &\mu'_{ij} = \Prob{\mid H_j(t)\mid^2 E_j(t-1)\geq  \sigma^2(2^{r_0}-1) \mid P(t-1) = i} \label{eq_prob} \\
%        &\text{and the mean received rate of (i,j) power-node pair $\mu_{ij} = r_0\mu'_{ij}$.}  \nonumber
       % & = \frac{e^{-\frac{p_{min}}{2\lambda P(t-1)\sigma_{dj}^2}}}{2\lambda P(t-1)\sigma_{dj}^2}\left\{\int_{0}^{B}e^{-\left(\frac{ \sigma^2(2^{r_0}-1)}{2u\sigma_{uj}^2} +\frac{u}{2\lambda P(t-1)\sigma_{dj}^2}\right)}du\right\} \nonumber \\  
        %& + \left\{e^{-\left(\frac{\sigma^2(2^{r_0}-1)}{2B\sigma_{uj}^2}\right)}e^{-\left(\frac{B+p_{min}}{2\lambda P(t-1)\sigma_{dj}^2}\right)}\right\}
%\end{align}
%which can be  computed numerically, where
$|G_j(t-1)|^2$ and $|H_j(t)|^2$  in $E_j(t-1)$ in \eqref{eqn:energy harvested} are exponentially distributed RVs with means $2 \sigma_{G_j}^2$ and $2 \sigma_{H_j}^2$, respectively. The variances $\sigma_{G_j}^2$ and $\sigma_{H_j}^2$ are obtained using the free-space path loss model as $\sigma_{x_j}^2=\frac{1}{2} 
\left(\frac{c}{4\pi f_{x_j}}\right)^2 d^{-\gamma}_j, x \in\{G,H\}$,
%\begin{align}
%\sigma_{x_j}^2=\frac{1}{2} 
%\left(\frac{c}{4\pi f_{x_j}}\right)^2 D^{-\gamma}_j, \quad x \in\{d,u\},
%\end{align}  
where  $c$ denotes the speed of light, $f_{x_j}$ for $x \in\{G,H\}$ is the carrier frequency of the signal to/from the node $j$, $d_j$ is the length of the link between the source and node $j$, and $\gamma$ is the path loss exponent. Moreover, the noise power $\sigma^2$ in \eqref{eq_O} is given by $\sigma^2=W \sigma_0^2$, where $W$ is the bandwidth and $\sigma_0^2$ is the noise power per Hz.   
For our numerical simulations, we assume a bandwidth $W=100$ kHz and noise power per Hz  $\sigma^2_0=-170$ dBm/Hz, that makes the total noise power $\sigma^2=-120$
%10^{-15}$ Watts
dBm. We assume carrier frequencies as $f_{G_j}=2.4$ GHz and $f_{H_j}=2.4+(10^{-3}\times j)$ GHz, the length $d_j=10+(3\times j)$ m, $\omega_j = 1/k$ for $j=1,2,..k$. Furthermore, we consider the path loss exponent $\gamma$ = 2.5, %the rate $r_0=0.1$ bits/channel use, 
the EH inefficiency coefficient $\lambda=0.5$, the minimum power $p_{\min}=-60$
%10^{-9}$ Watts 
dBm, the maximum battery capacity $b_{\max} \geq -40$ dBm,  and $\alpha=3$. %$10^{-7}$ Watts. 
For our EH setup, we consider the set of transmit powers as $\mathcal{P} = \{0,1,2,\dots,30\}$ in dBm. %$p_i = p_1 + (\frac{p_m - p_1}{m-1}) \times (i-1)$ $\forall i = 1,2,..,m$, where $p_1$ and $p_m$ are the lower and upper limits of the transmit powers, respectively and $m=10$.

%\vspace{-3mm}
We empirically evaluate the performance of our proposed algorithm \ref{alg:UCB} in terms of average EE and compare it with %for two experiments from the point of EE. %Experiment $1$ compares the behaviour of EE on different values of transmit power.
%Experiment $1$ compares the behaviour of EE on different values of rate $r_0$.
%Experiment $2$ compares the behaviour of EE on different number of nodes. We also compare EE of our algorithm with the 
a benchmark scheme without CSI. In the benchmark scheme without CSI the source always transmits with the maximum power to charge the EH nodes, i.e., it transmits with power $30$ dBm. We define the oracle scheme as the scheme based on the optimal policy which maximizes the energy efficiency of the system. The aim is our algorithm to learn the oracle scheme with time. %We define an oracle scheme where the source always transmits with the optimal power that maximizes the EE of the system. %has a priori knowledge of the best policy, i.e. always transmits with the optimal power, such that the EE of the system is maximized. 
We measure the performance of our algorithm for $T = 10^4$ time slots and the results are averaged over $1000$ repetitions. %The empirical results validate sub-linear bounds for our algorithm.

%\vspace{-3mm}
%\noindent
%\textbf{Energy Efficiency v/s  Transmit Power (in dbm):} \\
%The plot Fig. \ref{fig:ee_B} shows the impact of EE on increasing values of transmit power as %$[-3.01,0,6.99,10,16.99,20,26.99]$ (in dBm), 
%for varying number of nodes $(4,6,10)$. We find that for all number of nodes, EE satisfies the concave nature in transmit powers due to eq. \eqref{eqn:energy harvested}, and the transmit power $16.99$ dBm provides the maximum EE.
%\textbf{Energy Efficiency v/s Rate $r_0$ (in bits/channel):} \\
In Fig. \ref{fig:ee_vs_nodes}, we show the EE achieved with the proposed algorithm, the oracle scheme, and the benchmark scheme without CSI for different numbers of nodes $k =\{4,8,12\}$ and $r_0 = 0.1$ bpcu as a function of the number of time slots $n$. We find that the EE decreases as the number of nodes increases for a fixed number of transmit powers, as expected. As Fig. \ref{fig:ee_vs_nodes} shows, our algorithm achieves an EE that converges toward the EE achieved with the oracle. %converges towards its optimal transmit power. We carry out this experiment%Moreover, for number of nodes as $4,8,$ and $12$, the EE obtained using the benchmark are $0.09,0.07,$ and $0.05$ respectively. In contrast, the EE corresponding to the optimal transmit powers using UCB-EH are $0.64,0.32,$ and $0.21$, respectively, which are significantly high. As compared with the benchmark, our algorithm outperforms.
Moreover, our algorithm significantly outperforms the benchmark scheme without CSI for any $k$ and for any time slot.
% in the sense that for each number of nodes the optimal transmit power obtained using \ref{alg:UCB} is significantly higher as compared to the benchmark.
\vspace{-4mm}
\begin{figure}[H]
\centering
%\hspace{-2mm}
%\begin{subfigure}[b]{0.55\textwidth}
	\includegraphics[width=9.5cm, height = 4.3cm]{Figures/Original_Revised_compare_EE_weighted_nodes_oracle_benchmark_r0_0.1_10000_1001.pdf}
	\caption{Energy Efficiency v/s Time Slots.}
	\label{fig:ee_vs_nodes}
%\end{subfigure}
\vspace{-2mm}
\end{figure}
In Fig. \ref{fig:ee_r0}, we show the EE achieved with the proposed algorithm, the oracle scheme, and the benchmark scheme without CSI as a function of the rate $r_0$ when we have $k=5$ nodes. Initially, as we increase the value of $r_0$, more number of nodes can successfully transmit a codeword with rate $r_0$ to the source for a fixed transmit  power level at the source. As a result, the expected EE of the system increases and reaches its maximum point. But as $r_0$ increases further, more number of nodes fail to successfully transmit a codeword with rate $r_0$ to the source which will decrease the EE of the system. As Fig. \ref{fig:ee_r0} shows, our algorithm achieves an EE which is $52\%$ higher than the benchmark scheme without CSI and just $9\%$ lower than the oracle scheme. Moreover, to get the system's highest EE, our algorithm and the oracle scheme need a rate of $0.75$ bpcu, while the benchmark scheme without CSI requires $2$ bpcu to get the system's highest EE.
\vspace{-4mm}
\begin{figure}[H]
\centering
%\begin{subfigure}[b]{0.55\textwidth}
		\includegraphics[width=9.5cm, height = 3.8cm]{Figures/new_energy_efficiency_r_0_10000_1000_15.pdf}
    	\caption{Energy Efficiency v/s Rate $r_0$ (in bpcu).}
      	\label{fig:ee_r0}
%\end{subfigure}
%\caption{Empirical Performance of \ref{alg:UCB}}
\vspace{-2mm}
\end{figure}
In Fig. \ref{fig:ee_oracle}, we compare the EE of our scheme   with a benchmark scheme that has CSI knowledge of all channels for $k=8$. For a fair comparison, we have included in the  benchmark scheme  the cost of acquiring   CSI.  As can be seen from Fig. \ref{fig:ee_oracle}, the benchmark scheme with CSI  outperforms our algorithm only if the CSI cost is very small, i.e., less than -60 dBm in this example, which is not possible in practice since CSI estimation consumes a fair bit of energy.
\vspace{-4mm}
\begin{figure}[H]
	\centering
	%\addtocounter{figure}{-1}
	\includegraphics[width=9.5cm, height = 3.6cm]{Figures/Node_8_with_expense_Oracle_plot_0.1_10000_1000.pdf}
	%\includegraphics[width=0.5\linewidth]{Figures/Figure.png}
	\caption{\small{Energy Efficiency with and without CSI.}}
% 	A energy source with  $5$ energy harvesting nodes. The source can transmits one of the $3$ frequency bands.
	\label{fig:ee_oracle}
	%\vspace{-mm}
\end{figure}
\vspace{-2mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{figure}[H]
\centering
		\includegraphics[width=9.5cm, height = 4.5cm]{Figures/new_energy_efficiency_r_0_10000_1000_15.png}
    	\caption{Energy Efficiency v/s Rate $r_0$ (in bits/channel)}
      	\label{fig:ee_r0}
\end{figure}
\end{comment}

\vspace{-3mm}
%\textbf{Energy Efficiency v/s Number of Nodes:}\hspace{2mm} 
%\vspace{-3mm}

\begin{comment}
\newpage
\vspace{5mm}
\dg{My workings:-}

\textbf{We have to find the probability derivation of eq. 10}

\vspace{5mm}


\subsection{To find the distribution function of random variable $E$.}




\textbf{Proposition:} If $X \sim \mathcal{CN}(0, \sigma_{x}^2)$ (Complex Normal) then $|X|^2 \sim$ Exponential distribution $(mean = 2\sigma_x^2)$.

\begin{proof}
 Let $X = U + iV$, where $U, V \sim \mathcal{N}(0, \sigma_{x}^2)$, and they are independent.
 
 Therefore, $|X|^2 = U^2 +V^2$
 
 The cdf of $Y = U^2$,
 \begin{align}
     \Prob{Y \leq y} &= \Prob{-\sqrt{y} \leq U \leq \sqrt{y}} \nonumber\\
     & = \Prob{-\frac{\sqrt{y}}{\sigma_x} \leq Z \leq \frac{\sqrt{y}}{\sigma_x}} \qquad \text{where $Z = U/\sigma_x$} \nonumber\\
     & = 2\Phi\left(\sqrt{\frac{y}{\sigma_x^2}}\right) - 1  = F_{Y}(y) \label{eqn: cdf of Y}\\
     \intertext{Therefore, the pdf of $Y$,} \nonumber
     f_{Y}(y) &= 2\phi\left(\frac{\sqrt{y}}{\sigma_x}\right) \frac{1}{2\sigma_x \sqrt{y}} \nonumber\\
     & = \frac{1}{\sqrt{2\sigma_x^2} \Gamma(1/2)}e^{-\frac{y}{2\sigma_x^2}} y^{1/2 - 1} \nonumber\\
 \end{align}
Hence $Y= U^2 \sim Gamma(1/2, 2\sigma_x^2)$.

Similary, $V^2 \sim Gamma(1/2, 2\sigma_x^2)$.

Therefore, $|X|^2 = U^2 +V^2 \sim Gamma(1, 2\sigma_x^2)$

$\Rightarrow  |X|^2 \sim \text{Exponential Distribution (mean} = 2\sigma_x^2)$.

$\Rightarrow F_{|X|^2}(x) = 1 - e^{-\frac{x}{2\sigma_x^2}}$.
\end{proof}

%where $X \sim$ Exponential distribution with mean $2\sigma_{uj}^2$, i.e. $f_{X}(x) = \frac{1}{2\sigma_{uj}^2}\exp{\left(- \frac{x}{2\sigma_{uj}^2}\right)}$.

%For our problem,

%Let us define $H$, $G$, $E$ are random variables where , and $\lambda p(t) =a$. Here we consider $B, p_{min}, a,c > 0$.

%\newpage
\subsection{What is the distribution function of $E$ ?}

\begin{equation*}
    E =
    \begin{cases}
        0, & \text{if $aG \leq p$}\\
        aG - p, & \text{if $p < aG < B+p$} \\
        B, & \text{if $aG \geq B+p$}
    \end{cases}
\end{equation*}

Here $E$ takes two discrete values $0, B$ and is continuous in $(0,B)$.

For our problem, $ H \sim \text{Exponential Distribution (mean} = 2\sigma_{h}^2)$ and $G \sim \text{Exponential Distribution (mean} = 2\sigma_{g}^2)$ and the constants 

\vspace{3mm}

\textbf{The distribution of $E=E_{j}(t)$:}

\vspace{3mm}
For $G \leq \frac{p}{a}$, $ E =0$.

For $\frac{p}{a} < G < \frac{B+p}{a}$, $ E \in (0, B) \Rightarrow E \geq 0$.

For $G \geq \frac{B+p}{a}$, $E = B \Rightarrow E \text{ lies in the interval } [0,B]$ where ${0,B}$ are discrete and continuous in between $(0,B)$.

\begin{itemize}
    \item For $e =0$,
          \begin{align}
              \Prob{E=0} & = \Prob{G < \frac{p}{a}} \nonumber \\
              & = F_{G}\left(\frac{p}{a}\right) \nonumber
          \end{align}
    \item For $0 < e < B$,
          \begin{align}
              &\Prob{E \leq e}  = \Prob{E = 0} + \Prob{0 < E < e}\nonumber \\
              & = F_{G}\left(\frac{p}{a}\right) + \Prob{\frac{p}{a} < G < \frac{e + p}{a}} \nonumber \\
              & = F_{G}\left(\frac{p}{a}\right) + F_{G}\left(\frac{e + p}{a}\right) - F_{G}\left(\frac{p}{a}\right) \nonumber \\
              & = F_{G}\left(\frac{e + p}{a}\right) \nonumber
              \intertext{The pdf is given as,}\nonumber
              &f_E(e) = \frac{1}{2a\sigma_g^2}e^{-\left(\frac{e+p}{2a\sigma_g^2}\right)} \qquad \text{for $0 < e <B$} \label{eqn:pdf of E}
          \end{align}
    \item For $e=B$,
        \begin{align}
            \Prob{E =B} &=  \Prob{G \geq \frac{B+p}{a}} \nonumber \\
            &= 1 - F_G\left(\frac{B+p}{a}\right) 
        \end{align}
\end{itemize}

Therefore, the distribution function of $E$,

\begin{equation*}
    F_E(e) =
    \begin{cases}
        0, &\text{if $e < 0$}\\
        F_G\left(\frac{e+p}{a}\right), &\text{if $0 \leq e < B$}\\
        1, &\text{if $e \geq B$}
    \end{cases}
\end{equation*}



\subsection{We have to obtain $\Prob{HE \geq c}$.}

%Let us denote $c = \sigma^2(2^{r_0}-1)$.

The graph is plotted as below,

 \begin{figure}[H]
	\centering
	\includegraphics[width=0.9\linewidth]{Graph.png}
    \caption{Graph of $HE=c$}
    \label{fig:Graph}
\end{figure}


As $H \geq 0$ and $E \geq 0$, the random variable $HE \geq 0$.

Therefore, $\Prob{HE \geq c} = 1$ for $c=0$.

\vspace{5mm}

\textbf{\underline{ For $c>0$}}
\begin{align}
    & \Prob{HE \geq c} \nonumber \\
    &= \Prob{HE \geq c \mid E = 0}\Prob{E = 0} + \nonumber\\
   & \Prob{HE \geq c \mid 0 < E < B}\Prob{0 < E < B} + \nonumber\\
   &\Prob{HE \geq c \mid E = B}\Prob{E = B} \nonumber \\
   & = 0 + \int_{0}^{B}\Prob{H \geq \frac{c}{e}}f_E(e)de \nonumber\\
   &+ \Prob{H \geq \frac{c}{B}}\left(1 - F_G\left(\frac{B+p}{a}\right)\right) \nonumber \\
   & = \int_{0}^{B} e^{-\left(\frac{c}{2e\sigma_h^2}\right)}\frac{1}{2a\sigma_g^2}e^{-\left(\frac{e+p}{2a\sigma_g^2}\right)}de + \left\{e^{-\left(\frac{c}{2B\sigma_h^2}\right)}e^{-\left(\frac{B+p}{2a\sigma_g^2}\right)}\right\} \nonumber \\
   & = \frac{e^{-\frac{p}{2a\sigma_g^2}}}{2a\sigma_g^2}\left\{\int_{0}^{B}e^{-\left(\frac{c}{2e\sigma_h^2} +\frac{e}{2a\sigma_g^2}\right)}de\right\} \nonumber\\
   &+ \left\{e^{-\left(\frac{c}{2B\sigma_h^2}\right)}e^{-\left(\frac{B+p}{2a\sigma_g^2}\right)}\right\} \nonumber \\
    \intertext{The above integration solved through numerical simulation} \nonumber
\end{align}

\begin{equation*}
    \Prob{HE \geq c} =
    \begin{cases}
        1, &\text{if $c = 0$}\\
        \frac{e^{-\frac{p}{2a\sigma_g^2}}}{2a\sigma_g^2}\left\{\int_{0}^{B}e^{-\left(\frac{c}{2e\sigma_h^2} +\frac{e}{2a\sigma_g^2}\right)}de\right\} \\ + \left\{e^{-\left(\frac{c}{2B\sigma_h^2}\right)}e^{-\left(\frac{B+p}{2a\sigma_g^2}\right)}\right\}, &\text{if $c > 0$}
    \end{cases}
\end{equation*}

\vspace{5mm}
The above derivation is checked for mean(H) = 10 and mean(G) = 10. 
The simulation graph:

 \begin{figure}[H]
	\centering
	\includegraphics[width=0.9\linewidth]{fig_simulation_eq_10(matlab).jpg}
    \caption{Graph of $\Prob{HE \geq c}$}
    \label{fig:Graph}
\end{figure}


\newpage


\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%We computed computer simulations to evaluate the performance of the proposed algorithm \ref{alg:UCB} for two set of experiments. The first experiment compares the behaviour of regret on varying minimum sub-optimality gap where $\Delta_{min} = \min_{i \in m \setminus i^{*}} \Delta_{i}$. Whereas the second experiment compares the regret behaviours for different number of transmit powers and nodes. 

% \vspace{2mm}
%\noindent
%\textbf{Regret v/s Minimum sub-optimality gap:}\hspace{1mm} We plot in Fig. \ref{fig:deltaRegret} the impact of regret on different minimum sub-optimality gaps given as  $\Delta_{min} = (0.03, 0.04, 0.05, 0.06, 0.07)$. This validates the regret decreases as the minimum sub-optimality gap increases as proved theoretically.
 
% \begin{figure}[H]
%	\centering
%	\includegraphics[width=0.7\linewidth]{Figures/compareMinDelta_10000_1000.png}
 %   \caption{Regret v/s $\Delta_{min}$}
  %  \label{fig:deltaRegret}
%\end{figure}

%\vspace{-5mm}
%\textbf{Regret v/s Number of Powers and Nodes:}\hspace{2mm} We computed this experiment for different number of powers $(4,6,8)$and different number of nodes $(4,6,8)$. Fig. \ref{fig:regret_vs_power} indicates that the average regret increases as the number of powers increases for a fixed number of nodes, whereas, Fig. \ref{fig:regret_vs_nodes} indicates that the average regret remains almost equal for different number of nodes for a fixed number of powers. As per our theoretical analysis, the simulated results also verify that regret is dependent on both the number of powers and nodes.

%\vspace{-3mm}
%\begin{figure}[H]
%	\centering
%	\begin{subfigure}[b]{0.2\textwidth}
%		\includegraphics[width=\linewidth]{Figures/barPlot_Power_nodes4_new.png}
%    	\caption{Regret v/s Powers}
%   	\label{fig:regret_vs_power}
%	\end{subfigure}
%		\includegraphics[width=\linewidth]{Figures/barPlot_Nodes_Power8_new.png}
%		\caption{Regret v/s Nodes}
%		\label{fig:regret_vs_nodes}
%	\end{subfigure}
%	\caption{Empirical performance of \ref{alg:UCB}}
%	\label{fig:regret 1}
%\end{figure}




==> Energy Harvesting_Problem/introduction.tex <==
Wirelessly powered communication networks (WPCNs), where nodes can perform Energy Harvesting (EH), have recently drawn an upsurge in interest as a possible technology for next generation wireless networks. EH helps to enhance the life of wireless nodes by continuously charging their batteries either by scavenging energy from the ambient atmosphere or from a dedicated energy source. When a dedicated energy source is used for energy transmission, the amount of energy it emits has to be appropriately calibrated. In the one hand, high-power emissions may result in energy wastage due to the fundamental limitations of the amount of energy EH devices can harvest. On the other hand, low-power emissions may result in EH devices not being able to harvest enough energy. %On the one hand, emitting high power may result in wastage of energy due to the fundamental limitations in the amount of energy devices can harvest, and on the other hand, emitting low power may result in devices not being able to harvest enough energy. 
It is thus important that the energy source transmits with the right amount of power. As a result, the metric Energy Efficiency (EE), measured in bits-per-joule, has drawn considerable attention as an essential performance metric for optimizing the transmit power in WPCNs. Motivated by this, our goal in this paper is to develop an algorithm that learns the optimal power level of an energy source that maximizes the EE in WPCNs. %and  in both academia and industry .  Both Simultaneous Wireless Information and Power Transfer (SWIPT) systems, which characterizes fundamental trade-offs in simultaneous WET and WIT with the same transmitted signal, and Wireless Powered Communication Network (WPCN) where wireless terminals communicate using WET energy, are two main paradigms of research.

%A “harvest-then-transmit” protocol for WPCNs was developed in \cite{ju2013throughput} that jointly optimized the time allocated to the base station for downlink (DL) WET and the users for uplink (UL) WIT to maximize the system throughput. But the energy consumption for both energy transfer and information transmission was not considered. Nowadays, due to dramatic increase in energy consumption of wireless communications, the energy costs and carbon footprints of communication systems increased significantly. The performance metric "Energy Efficiency (EE)”, measured in bits-per-joule [2-6], has drawn a considerable attention in this scenario, which is widely used in WPCNs.

%Several papers have investigated EE in WPCN with simultaneous wireless information and power transfer (SWIPT) in various systems like .  \cite{shi2015energy,ng2013wireless,wu2016user,wu2014resource,guo2017energy}. Specifically, the multiuser multiple-input-single-output system y jointly optimizing the transmit beamforming and the receive power splitting thresholds. The authors in \cite{ng2013wireless} propose a resource allocation algorithm for maximizing the EE of an Orthogonal Frequency-Division Multiple Access (OFDMA) system employing SWIPT by optimizing the power allocation, subcarrier allocation, and the user scheduling. In \cite{wu2016user}, the authors propose a user-centric resource allocation algorithm that maximizes the weighted sum of the user's EEs by jointly optimizing the time allocation and the power control of the downlink wireless energy transmission (WET) and the uplink wireless information transmission (WIT). The authors in \cite{wu2014resource} develop a joint transmitter and receiver optimization of the EE of OFDMA systems by considering the effects of active subcarriers and users on the system. The authors in \cite{guo2017energy} study the energy-efficient SWIPT in mobile wireless sensor networks that consider the minimum individual and system data rate requirements of the receivers, the minimum required power transfer, and the maximum system power consumption. 

Several authors have investigated EE of various WPCNs. For example, the authors in \cite{shi2015energy} study the maximization of EE in multi-users multiple-input-single-output systems with Simultaneous Wireless Information and Power Transfer (SWIPT). The authors in \cite{ng2013wireless} study EE of Orthogonal Frequency Division Multiple Acesss (OFDMA) systems employing SWIPT. The authors in \cite{wu2016user}, maximize the weighted sum of the user's EEs by jointly optimizing the used power for downlink wireless energy transmission (WET) and for uplink wireless information transmission (WIT). Similar joint transmitter and receiver optimization of EE of OFDMA systems taking into account the effects of active subcarriers and users is studied in \cite{wu2014resource}. The authors in \cite{guo2017energy} study the EE of SWIPT in mobile wireless sensor networks considering the minimum individual and system data rate requirements of the receivers, the minimum required power transfer, and the maximum system power consumption. 

The works \cite{shi2015energy}-\cite{guo2017energy}, as well as others in the literature, study EE in WPCNs assuming that the channel state information (CSI) is known at the receivers and/or the transmitters. However, acquiring CSI consumes energy, which diminishes the EE of the system. As a result, we propose a learning algorithm that maximizes the EE of the system without any CSI knowledge. Specifically, we consider a WPCN where the energy source transmits energy to EH nodes and the nodes use the harvested energy to transmit information back to the energy source at a fixed rate. The energy source then tries to decode the received codewords and observes which nodes were successful in their transmission. Using this limited information regarding the successful decoding of received codewords, the source learns which power level to use in order to maximise the EE of the system. % for energy transmission in the next time slot. 
To this end, we model the problem as a stochastic multi-armed bandits problem and %\sout{ propose a corresponding solution.} 
develop a learning algorithm to optimize EE. %where the goal of the energy source is to learn a power level that maximizes the EE of the system defined as the weighted sum rate received from the nodes per unit transmit power.%where the energy source is the learner and the power levels available to transmit energy are the arms. 

Learning algorithms in WPCN were investigated recently in \cite{luo2019learning} and \cite{min2019learning}. The authors in \cite{luo2019learning} propose reinforcement learning (RL) to investigate the tradeoff between EE and quality of service parameters, such as transmission delay, in device-to-device communications underlaying cellular networks. The authors in \cite{min2019learning} propose a RL based offloading policy for EH IoT devices to select the edge devices for computationally intensive applications. These learning algorithms require that the devices either have CSI or know additional information such as the available battery power, tasks which are hard to realize in practice and also that diminish the EE. n this paper, we adopt the multi-armed bandit framework for solving the EE problem since it enables us to establish theoretical guarantees on the performance of our algorithm. Thereby, we propose an Upper Confidence Bound (UCB) based learning algorithm using which the energy source maximizes the EE without any CSI and only based on whether a received codeword was successfully decoded or not. To the best of our knowledge, maximizing the EE of a WPCN by optimizing the power selection strategy without CSI knowledge has not been studied previously. %\sout{On the other hand, system model considered in this paper is applicable to wireless sensor networks.}

%The remainder of this work is organized as follows. Sec. \ref{sec:system_model} introduces the system model. In Sec. \ref{sec:problem_formulation} we formulate the EE maximization problem as a multi-armed bandit problem and propose an algorithm that maximizes EE and give its performance guarantees. % and introduce stochastic Multi-Armed Bandits (MAB) set up for the problem in Sec. \ref{sec:solution}. We propose Upper Confidence Bounds (UCB) based algorithm, named as \ref{alg:UCB}, along with its performance guarantee for the new set up in Sec. \ref{sec:algorithm}.
%We empirically validate the performance of our algorithm %named as \ref{alg:UCB} on practical set up 
%in Sec. \ref{sec:experiment}, and conclude the paper in Sec. \ref{sec:conclusion}.
%\vspace{-2mm}

==> Energy Harvesting_Problem/problem_formulation.tex <==
In the following, we formulate the problem and develop a learning algorithm to maximize the EE in the WPCN.
\vspace{-2mm}
\subsection{Problem Setting}
\label{sec:problem_setting}
\input{problem_setting}
	
\subsection{Notation}
\label{sec:solution}
\input{solution}

\subsection{The Proposed Algorithm}
\label{sec:algorithm}
\input{algorithm}

==> Energy Harvesting_Problem/problem_setting.tex <==
As we increase the transmit power of the source, the amount of energy harvested by the nodes increases only to a certain point and then saturates due to  \eqref{eqn:energy harvested}. As a result, further increase in the transmit power of the source will not increase the weighted sum rate received at the source given by \eqref{eqn:sum_data_rate}, thereby leading to a wastage of energy. Hence, there must be some optimal power level which maximizes the weighted sum rate per energy spent. %Even before such saturation occurs, there exists a transmit power of the source that maximizes the weighted sum rate received at the source with the minimum possible transmit power by the source. % we define sum rate per unit power transmitted in the long run. Specifically, 
To investigate this point, we define the EE as a ratio between the weighted sum rate received at the source and source's transmit power over $n$ time slots given as
%Energy Efficiency (EE) defined as follows: 
\begin{align}
  %EE=\lim\limits_{n\to\infty}\frac{1}{n}\sum\limits_{t=1}^{n}\sum_{j=1}^{N}\frac{R_{j}(t+1)}{P(t)} \quad \\
  %\max\limits_{P(t) \in \mathcal{P}, \forall t}
 %\max\limits_{P(t) \in \mathcal{P}, \forall t } 
 EE(n) = \frac{1}{n}\sum_{t=1}^n\sum_{j=1}^k \frac{\omega_jR_j(t+1)}{P(t)}.
\end{align} 
Our goal is to identify a fixed power level that maximizes the expected EE, i.e., we solve the following optimization problem
\begin{align}
\arg\max\limits_{p \in \mathcal{P}}\EE{EE(n) \mid P(t) = p, \; \forall \; t}\label{eqn:NTP}.
\end{align}
  %EE(n) =  \frac{1}{n}\sum_{t=1}^n  \max\limits_{P(t) \in \mathcal{P}, \forall t }\sum_{j=1}^k \frac{R_j(t+1)}{P(t)}
 %Notice that we seek to identify the power that maximizes EE when used in all time slots. 
 The rationale for seeking a fixed power level in all time slots is because the source does not have CSI and hence adapting the power levels in each time slot is not useful. The only information available to the source is whether a received codeword from a given node was successfully decoded or not. %s' transmission it could successfully decode. %Obviously, this optimization problem can be solved relatively easy if the CSI is known, i.e., if $G_j(t)$ and $H_j(t)$ are known $\forall j$ and $\forall t$. However, acquiring the CSI consumes energy and is therefore not energy efficient. As a result, in this paper we assume that the source does not have any CSI knowledge nor knows the distribution of the CSI a priori. %Note that the amount of energy harvested by each node is random due to the stochastic nature of the fading channels gains. Also, due to practical limitations, they will not the amount of energy harvested by the nodes in each time slot. Hence the source cannot even estimate the parameters of the distribution. 
%Instead, the only information the source has is whether a codeword transmitted from a given node was correctly decoded or not. 
Based on this limited information, we derive a strategy for the source to learn the optimal power that maximizes the expected value of the EE defined by \eqref{eqn:NTP}. %We model our problem as a MAB problem where the goal is to identify an optimal transmit power such that the EE, defined as \eqref{eqn:NTP}, is maximized.
\vspace{-3mm}

==> Energy Harvesting_Problem/solution.tex <==
We refer to each power in the set $\mathcal{P}$ simply by its index.  Let $\boldsymbol{R}(t)=\{R_1(t), R_2(t),...,R_{k}(t)\}$ denote the vector of received rates at the source in time slot $t$, where $R_j(t)$ is the received rate from node $j$, given by \eqref{eqn: received rate}. Note that the vector $\boldsymbol{R}(t)$ depends on the energy harvested by the nodes in the previous time slot $t-1$. At $t=1$, $R_j(1)=0, \forall j$, as the nodes do not have any energy harvested from $t=0$. %For each $n$, the random sequence $\{R_n(t)\}_{t\geq 1}$ is independently and identically distributed. Decision of the source in each round is the power level for energy transmission and the feedback it receives is rate achieved for each node. 
Let the history at the source in time slot $t$ be defined as $\mathcal{H}(t):= \left\{(P(1),\boldsymbol{R}(1)),(P(2),\boldsymbol{R}(2)),..,(P(t),\boldsymbol{R}(t))\right\}$ with $\mathcal{H}(0) = \phi$. The power selection policy of the source denoted by $\Pi = \left\{\pi(t)\right\}_{t=1}^{\infty}$ is a sequence of maps $\pi(t):\mathcal{H}(t-1) \rightarrow \mathcal{P}$. % which denotes the power selected by the source in time slot $t$ given the history $\mathcal{H}(t-1)$.
Our goal is to find a policy that maximizes the expected EE of the system given by \eqref{eqn:NTP}. To this end, we set up the problem as a Multi-Armed Bandits (MAB) problem, where the source is the learner and the set of transmit powers at the source constitute the arms.

%For a transmit power selected by the source, the amount of energy harvested and the corresponding rate received from each node are i.i.d. across the time slots. 
Let $R_{j}^i(t)$ denote the rate received at the source from node $j$ in time slot $t$, when the transmit power of the source in time slot $t-1$ was $P(t-1)=i$. For each node $j$ and power $i$,  the random process $\left\{R_j^i(t)\right\}_{t\geq 2}$ is an independent and identically distributed (i.i.d.) process with a mean denoted by $\mu_{ij}$ and given by $\EE{R_j(t+1)|P(t)=i} = \mu_{ij}$. We denote the power that maximizes the expected EE by $i^{*}$ and denote the corresponding optimal expected EE by $\mu_{i^{*}}$, where 
\begin{align}
    i^{*} = \argmax_{i\in m}\sum_{j=1}^{k}\frac{\omega_j\mu_{ij}}{p_i} \quad \text{and}\quad \mu_{i^{*}} = \sum_{j=1}^{k} \frac{\omega_j\mu_{i^*j}}{p_{i^*}}.
    %\vspace{-1mm}
\end{align}
We define the expected regret that evaluates the performance gap between the proposed strategy and the optimal power selection strategy on average over $n$ time slots as $\Regret_{n} = n\mu_{i^{*}} - \sum_{t=1}^{n} \sum_{j=1}^{k}\omega_j\EE{\frac{\mu_{I_{t}j}}{p_{I_{t}}}}$,
%\begin{align}
%\label{regret}
%    \Regret_{n} = n\mu_{i^{*}} - \sum\limits_{t=1}^{n} \sum\limits_{j=1}^{k}\EE{\frac{\mu_{I_{t},j}}{p_{I_{t}}}}
%\end{align}
where $I_t$ is the power index selected in time slot $t$ and $p_{I_t}=P(t)$ is the associated transmit power. %The selection of $P(t)$, or $I_t$, could depend on the past stochastic observations $\left\{\boldsymbol{R}(2), \boldsymbol{R}(3),\dots,\boldsymbol{R}(t-1)\right\}$ and the expectation is taken with respect to this randomness. 
Hence, maximizing the average EE is equivalent to designing a learning algorithm that minimises the expected regret by learning the optimal power level at the source.

%and asymptotically leads to zero regret as $n \rightarrow \infty$.% We say a policy learns the environment if $\Regret_{n}/n \rightarrow 0$ as $n \rightarrow \infty$, i.e., the learned policy gives the same performance asymptotically as the best possible policy. %We will develop a upper confidence bound (UCB) based policy with sub-linear regret. 
\vspace{-2mm}

==> Energy Harvesting_Problem/system_model.tex <==
We consider a system model comprised of an energy source, referred to as the source, and $k$  EH wireless nodes, referred to as the nodes. The source and the nodes employ frequency-division duplex (FDD)\footnote{Alternatively, we can also assume that the source and the nodes employ time-division duplex (TDD) on $k+1$ time slots in order to avoid interference.} on $k+1$ dedicated channels where each channel occupies a different frequency band. Specifically, the source radiates energy on its dedicated channel, which is then harvested by the nodes and used to transmit information back to the source on their respective dedicated channels, cf. Fig. \ref{fig:Model}. Note that since FDD is used, interference does not occur. The source also serves as a receiver of information. We assume that the dedicated channels are flat-fading channels with channel gains that are constant in each time slot and change independently from one time slot to the next. Let $G_{j}(t)$ denote the complex-valued channel gain between the source and node $j$ in time slot $t$ on the channel dedicated for energy transmission, where $G_{j}(t)\sim\mathbb{CN}\{0,\sigma_{G_j}^2\}$, i.e., complex Gaussian distributed with mean zero and variance $\sigma^2_{G_j}$. Let $H_j(t)$ denote the complex-valued channel gain between node $j$ and the source in time slot $t$ on the channel dedicated for information transmission by node $j$, where $H_j(t)\sim\mathbb{CN}\{0,\sigma_{H_j}^2\}$.  
We also assume that the received signal at the source is corrupted by complex zero-mean additive white Gaussian noise (AWGN) with variance $\sigma^2$.

The source has a set of $m$ powers\footnote{The proposed algorithm works also with a continuum of power,  provided we quantize the continuous power into discrete power. Then, the proposed algorithm will learn the optimal discrete power that is close to the optimal continuous power.} denoted by  $\mathcal{P}=\{p_1, p_2,\dots,p_m\}$. In each time slot $t$, the source can select any power in $\mathcal{P}$ to transmit energy. Let $P(t) \in \mathcal{P}$ denote the power selected in time slot $t$. The amount of energy harvested by node $j$ in time slot $t$ from power $P(t)$, denoted by $E_{j}(t)$, is given by
\begin{align}
\label{eqn:energy harvested}
    E_{j}(t)=\min\{b_{\max},\max\left(0,\lambda P(t) |G_{j}(t)|^2 - p_{\min}\right)\},
\end{align}
where $p_{\min}$ is the minimum required power for each node to operate, $0 \leq \lambda <1$ is the EH inefficiency coefficient, and $b_{\max}$ is the maximum capacity of the battery of the nodes. We assume that the nodes use the entire energy harvested in time slot $t-1$ for information transmission in the next time slot $t$. Each node transmits information using a capacity-achieving codeword with rate $r_0$. %and transmitting it with power $P_j(t-1)$. 
The received rate at the source from node $j$ in time slot $t$ is denoted by $R_j(t)$ and is given by
\begin{align}
\label{eqn: received rate}
    R_{j}(t) & =O_{j}(t) r_0,
\end{align}
where $O_j(t)$ is a binary variable that models success or failure of the decoding of the codeword of node $j$ at the source, given as
%\vspace{-3mm}
\begin{align}\label{eq_O}
    O_{j}(t) &=\left\{\begin{array}{ll}
        1      & \textrm{if } \log_2\left(1+\frac{E_{j}(t-1) |H_j(t)|^2}{\sigma^2}\right)> r_0  \\
        0      & \textrm{otherwise}.  
 \end{array}
 \right.
 \end{align}
Using $R_j(t),\forall j$, we can define the weighted sum rate received at the source in time slot $t$ as
%\vspace{-2mm}
\begin{align}
R_{sum}(t) =\sum\limits_{j=1}^{k}\omega_jR_j(t),\label{eqn:sum_data_rate}
%\vspace{-2mm}
\end{align}
where $0 \leq \omega_j \leq 1, \forall j$, and $\sum_{j=1}^k\omega_j = 1$. The weights $\omega_j, \forall j$, are used to give different priorities to the users. %From Eq.~\ref{eq_O}, note that $R_j(t)$ denotes the rate for node $j$ in round $t$ from the energy it harvested in round $t-1$.
%\vspace{-4mm}
\begin{figure}[!h]
	\centering
	\includegraphics[width=9cm, height = 4cm]{Figures/Figure_new_edit.pdf}
	%\includegraphics[width=0.5\linewidth]{Figures/Figure.png}
	\caption{\small{Energy Harvesting setup. Refer \cite{CST2014_wirelessnetwork_LuXiaoPingDusit} for a detailed architecture.}}
% 	A energy source with  $5$ energy harvesting nodes. The source can transmits one of the $3$ frequency bands.
	\label{fig:Model}
	\vspace{-4mm}
\end{figure}
%\vspace{-1cm}
%and the amount of energy harvested by the $n$-th EH node for $i$-th transmit power $P_{i_{t}}$ selected at round $t$ is given as,
%\begin{align*}
%    E_{i,n}(t)=\min\{B,\max\{0,\mu P_{i_{t}} %|g_{n}(t)|^2\}-P_C\}
%\end{align*}
%Hence, $O_{j}(t)$ is a binary variable which takes the value $O_{j}(t)=1$ if the codeword transmitted by the $j$-th node can be decoded successfully at the source and takes the value $O_{j}(t)=0$ if the decoding is unsuccessful. 

% We assume that the energy source can choose its transmit power from a discrete set of transmit powers, given as
% \begin{align}
%     \mathcal{P}=\{P_1, P_2, ...,P_L\}.
% \end{align}
% Hence, $P_{i_{t}}\in \mathcal{P}$ must hold for all $t=1,2,...,T$, where $T$ is the total number of time slots.
